How to Split: the Effect of Word Segmentation on Gender Bias in Speech Translation

Having recognized gender bias as a major issue affecting current translation technologies, researchers have primarily attempted to mitigate it by working on the data front. However, whether algorithmic aspects concur to exacerbate unwanted outputs remains so far under-investigated. In this work, we bring the analysis on gender bias in automatic translation onto a seemingly neutral yet critical component: word segmentation. Can segmenting methods influence the ability to translate gender? Do certain segmentation approaches penalize the representation of feminine linguistic markings? We address these questions by comparing 5 existing segmentation strategies on the target side of speech translation systems. Our results on two language pairs (English-Italian/French) show that state-of-the-art sub-word splitting (BPE) comes at the cost of higher gender bias. In light of this finding, we propose a combined approach that preserves BPE overall translation quality, while leveraging the higher ability of character-based segmentation to properly translate gender.

==> altenativa_finale.tex <==
Following these considerations, it appears that the conventional vision separating the two components’ activity in encoder-decoder architectures does not apply. In fact, although the 
%%Char and BPE
two
decoders do not interact with one another in the Multitask model, the system is nonetheless benefiting from Char’s attested ability to handle gender translation. As such, the chosen segmentation technique does not merely seem to determine a model’s improved capacity to extract %source 
%gender information in the encoder, and then render it into the target language. Rather, the target word segmentation might directly influence the gender information expressed and retained in the input’s internal representation, which is then leveraged in translation.

==> intro-versionilunghe.tex <==
APPUNTI part 3

are feminine forms longer in Must-SHE?
→ yes. (see sheet MuST-SHE analysis)
questo è il caso del quasi 15percent delle forme femminili italiane e quasi 95% di quelle francesi in termini di tokens
differenze si spiegano in termini di caratteristiche della singola lingua. 

are femine forms less frequent in MuST-C?
we calculate the frequency of MuST-SHE feminine vs masculine forms in MuST-C
(n.b. non usiamo morphological analyzer generico per evitare rumore → potrebbe sbagliare e soprattutto individuare forme femminili non human-related. Questo può succedere anche con parole di MuST-SHE ma rischio ridotto perchè sono largamente human-related (e.g. professional nouns, human referring adjectives..)

→ yes, feminine forms are less frequent in both French and Italian around 86-87 percent of the cases

N.B. most of the cases in which femine gender forms are more frequent are either gender-exclusive (e.g. incinta) or controversial (e.g. seccata, violentate, terrorizzata…)

N.B alcuni casi di parole funzione non sono indicativi, e.g. articolo la occorre più frequentemente, ma perché compete con due controparti maschili (il \& lo)

QUESTI RISULTATI CI PERMETTONO DI CONFERMARE CHE IL PROBLEMA DELLA TRADUZIONE DEL GENERE PUO’ ESSERE INQUADRATO COME UN PROBLEMA LEGATO ALLA LUNGHEZZA DELLE SEQUENZE DI PAROLE A FORMA FEMMINILE E DI PAROLE MENO FREQUENTI. 













\section{Introduction ACCORCIATA}

The widespread use of language technologies has motivated growing interest on their social impact \cite{hovy-spruit-2016-social,blodgett-etal-2020-language}, with  gender \cite{costa-nature, sun-etal-2019-mitigating} and other demographic biases \cite{kiritchenko-mohammad-2018-examining,sap-etal-2019-risk} representing the major causes of concern. As regards gender bias, focused evaluations have shown that both machine translation (MT) and speech translation (ST) systems do in fact perpetuate stereotypical gender associations \cite{Prates2018AssessingGB, stanovsky-etal-2019-evaluating, costa2020evaluating}, %\cite{costajussà2020evaluating} 
 overproducing masculine forms in their outputs \cite{bentivogli-2020-gender,gaido-etal-2020-breeding}.  While tackling such issues requires a long-term multidisciplinary commitment \cite{criado2019invisible,Ruha,d2020data}, most works have identified \textit{data} as the primary reason for gender bias. Accordingly,  many  pointed out the quantitative \cite{broadcast, vanmassenhove-etal-2018-getting} misrepresentation of gender groups in existing datasets, 
%and focused
focusing
on the development of data-centred mitigating techniques like counterfactual data augmentation \cite{zmigrod-etal-2019-counterfactual,lu2020gender} or on the creation of gender-balanced corpora \cite{saunders-etal-2019-domain, costa-jussa-de-jorge-2020-fine}. 

Data, however, represent only one aspect of the bias problem \cite{shah-etal-2020-predictive}, which should also be  viewed through the lens of the trade-offs between architectural choices,  overall output quality and  fairness. Along this direction, few inquiries  devoted attention to model components  concurring to exacerbate  the problem \cite{vanmassenhove-etal-2019-lost}. From an algorithmic perspective, recent studies demonstrated that architectural choices  do impact gender translation \cite{costa-jussa-etal-2020-multilingual}, and that ``taken-for-granted''  approaches,  like the choice of beam search over sampling, may come with high overall translation quality in terms of BLUE scores, but are actually detrimental when it comes to gender bias \cite{roberts2020decoding}.

Along  this line,  we focus on another core  aspect of neural MT: word segmentation. Byte-pair encoding (BPE) \cite{sennrich-etal-2016-neural} represents the state-of-the-art and has recently shown to yield higher results compared to character-based segmentation also in ST \cite{di-gangi-2020-target}. But does this hold true for gender translation as well? 
%Do the BPE advantages (i.e. the representation of an open vocabulary through a fixed-size vocabulary of character sequences) come at the cost of higher system bias? 
%
%Are there better alternative methods 

The above question is particularly relevant when dealing with  with grammatical gender languages, like French and Italian, where gender agreement is an extensive semantic and morpho-syntactic phenomenon \cite{Hockett:58,Corbett:91} marked by different feminine and masculine morphological inflections on multiple parts of speech. Moreover, such languages often exhibit comparatively complex feminine forms, derived from the masculine ones by means of additional suffixes (e.g. en: \textit{professor}, it: \textit{professor\underline{e}} vs. \textit{professor\underline{essa}}) \cite{pappas4gender}. In light of the above, purely statistical segmentation methods could be unfavourable for gender translation, as they  can break the morphological structure of words and thus lose relevant linguistic information \cite{ataman-2017-lmvr}. In terms of data distribution, instead, as women are under-represented in our corpora, so most likely are their referential linguistic expressions of gender. Consequently, since stochastic tokenizers proceed by merging word fragments that co-occur more frequently while  rarer combinations are left unmerged, there is the concrete risks that sparser feminine-marked words would result in less compact sequences of tokens (e.g. en: \textit{described}, it:  \textit{des@@ critt\underline{o}} vs. \textit{des@@ crit@@ t\underline{a}}). In light of such typological and distributive conditions, is it possible that because of statistical but linguistically-unmotivated and longer sequence of tokens, with each additional token bringing more uncertainty with respect to their masculine counterparts, feminine gender might results less probable and harder to predict?

We address such questions by implementing different families of segmentation approaches employed on the decoder side of translation models built on the same training data. By comparing the resulting models both in terms of overall translation quality and gender accuracy, we explore whether a so far considered irrelevant  aspect like  word segmentation can  actually favour or hinder gender translation.  Accordingly, our main contribution is the first comprehensive analysis of the results obtained by 5 popular segmentation techniques for two language directions (English/Italian, English-French). 
%Additionally, we integrate our evaluation with more informative diagnosis on two aspects interacting with the segmentation's gender performance: tokenized sequence length and words frequency.
We find that so far unnoticed variations in compression techniques do have an impact on gender bias and are a source of disproportionate generation of masculine forms.  Consistently, our experiments shows that there is a trade-off between higher BLUE scores for BPE \cite{sennrich-2017-how-grammatical} and character models' higher ability to  generalize the morphology of sparser feminine forms and better translate gender. Our study also implicates that further advances for proper gender translation may need to take into account typological differences across languages and focus on language-specific subword generation algorithms. 







\section{Introduction ORIG, TOO LONG}

Propelled by progress in the field of 
%BEA:
%machine
%MN:
deep
learning, language technologies have attested notable and rapid quality improvements in recent years. Having entered widespread use, however, their social impact has become a growing concern \cite{hovy-spruit-2016-social,blodgett-etal-2020-language}, with raising evidence of systems being affected by gender \cite{costa-nature, sun-etal-2019-mitigating} and other demographic biases \cite{kiritchenko-mohammad-2018-examining,sap-etal-2019-risk}. 

%BEA:
%Indeed, gender 
%MN:
Gender
bias concerns automatic translation, too. Focused evaluations have shown that both Machine Translation (MT) and Speech Translation systems do in fact perpetuate stereotypical gender associations \cite{Prates2018AssessingGB, stanovsky-etal-2019-evaluating} %\cite{costajussà2020evaluating} 
and overproduce masculine forms in their outputs \cite{bentivogli-2020-gender,gaido-etal-2020-breeding}.
%\sout{}
While tackling such issues requires a long-term multidisciplinary commitment \cite{criado2019invisible,Ruha,d2020data}, the community has currently put effort into exposing such adverse asymmetries and trying to mitigate them.

Most works have %generally 
identified data as the primary, if not only, reason for gender bias. Accordingly, several studies have pointed out the 
%hown the qualitative  and 
quantitative \cite{broadcast, vanmassenhove-etal-2018-getting} misrepresentation of gender groups in datasets, and focused on the development of data-centred mitigating techniques, like counterfactual data augmentation \cite{zmigrod-etal-2019-counterfactual,lu2020gender} or the creation of gender-balanced corpora \cite{saunders-etal-2019-domain, costa-jussa-de-jorge-2020-fine}. %While rethinking our data is a complex issue and relevant issue  that should be pu into its social, cultural and relation context \cite{bender,rawdata}

%BEA:
%However, data are not the only cause for bias \cite{shah-etal-2020-predictive}, 
%%%and comparatively little attention has been given to other models components that concur to exacerbate the problem. 
%with only few inquiries giving attention to other models components that concur to exacerbate the problem \cite{vanmassenhove-etal-2019-lost}.
%MN:
Although data are not the only cause for bias \cite{shah-etal-2020-predictive}, only few inquiries have given attention to other model components that concur to exacerbate the problem \cite{vanmassenhove-etal-2019-lost}.
From an algorithmic perspective, recent studies demonstrated that architectural choices 
%MN:
%in Multilingual MT 
do impact gender translation \cite{costa-jussa-etal-2020-multilingual}, and ``taken-for-granted''  approaches,  like the choice of beam search over sampling, may come with high overall translation quality in terms of BLUE scores, but are actually detrimental when it comes to gender bias \cite{roberts2020decoding}. 
Along the same line,  byte-pair encoding (BPE) \cite{sennrich-etal-2016-neural} represents the state-of-the-art compression algorithm in MT, and recently showing to achieve higher general results with respect to character-based segmentation also for ST \cite{di-gangi-2020-target}. But does this hold true for gender translation as well?

From a structural perspective, in languages with grammatical gender like French and Italian, gender agreement is an extensive semantic and morphosyntactic phenomenon \cite{Hockett:58,Corbett:91}, marked by different feminine and masculine morphological inflections on multiple parts of speech. Moreover, such languages often exhibit comparatively complex feminine forms, derived from the masculine ones by means of an additional suffixes (e.g. en: \textit{professor}, it: \textit{professor\underline{e}} vs. \textit{professor\underline{essa}}) \cite{pappas4gender}. In light of the above, purely statistical segmentation methods could be unfavourable 
%limiting? damaging?
for gender translation, as they 
%tokenize into linguistically-unmotivated unts and can thus
can break the morphological structure of words and thus lose relevant linguistic information \cite{ataman-2017-lmvr}. In terms of data distribution, instead, as women are under-represented in our corpora, so most likely are their referential linguistic expressions of gender. Consequently, since stochastic tokenizers proceed by merging words fragments that co-occur more frequently while leave rarer combinations are left unmerged, there is the concrete risks that sparser feminine-marked words would result in less compact sequences of tokens (e.g. en: \textit{described}, it:  vs. \textit{des@@ critt\underline{o}} vs. \textit{des@@ crit@@ t\underline{a}}). 

In light of such typological and distributive conditions, is it possible that because of statistical but linguistically-unmotivated and longer sequence of tokens, with each additional token bringing more uncertainty with respect to their masculine counterparts, feminine gender might results less probable and harder to predict?

In this work, we address such questions by implementing different families of segmentation approaches employed on the decoder side of translation models trained with the same type and amount of data. Their performance is compared both in terms of overall translation quality  as well an gender accuracy on the  gender-sensitive MUST-SHE benchmark \cite{bentivogli-2020-gender}. Our purpose is explore whether so far considered irrelevant, technical parameter like splitting algorithms can  actually favour or hinder gender translation. Accordingly, our main contribution is the first comprehensive analysis of both MT and ST models of 5 popular segmentation techniques designed to measure whether they have an impact on the extent of gender bias for two language-pairs (English/Italian, English-French). Additionally, we integrate our evaluation with more informative diagnosis on two aspects interacting with the segmentation's gender performance: tokenized sequence length and words frequency. 

We find that so far unnoticed variations in compression techniques do have an impact on gender bias and are a source of disproportionate generation of masculine forms. 
Consistently, our experiments shows that there is a trade-off between higher BLUE scores for BPE
\cite{sennrich-2017-how-grammatical} and character models' better ability to properly translate gender and generate feminine forms. Our examinations expose that character level splitting better generalizes to the morphology of sparser feminine forms. This study also implicates that further advances for proper gender translation may need to take into account typological differences across languages and focus on language-specific subwords generation. 




%or shed more light on the inner mechanism of opaque models \cite{vig-belinkov-2019-analyzing,bau2018identifying}. In fact, 

 %Closest to our intent are the works by (Costa Jussà et al, 2020) - which investigates the role different architectural designs play in gender bias in Multilingual MT - and (Roberts et al, 2020) proving that beam search is comparatively with sampling more biased toward the generation of more frequent (masculine) pronouns. In both works, it has been shown while “taken-for-granted” approaches, like -respectively - the use of Transformer architecture or beam search, improve overall translation quality in terms of BLUE scores, they are disadvantaged when it comes to gender bias. 


% Similarly, the BPE compression method is the MT state-of-the-art approach, and has been recently proved to be the highest-quality segmentation technique in ST as well (Di Gangi et al, 2020). But does it hold true for gender translation as well?



% Automatic Translation has been shown to exhibit gender bias. This holds true for both MT and ST, although to different extent and displaying different limits and potentialities (Bentivogli et al 2019, Gaido et al 2020, Costa-Jussà et al, 2020) 
% Although tackling gender bias in language technologies requires a long-term multidisciplinary work in education, society and politics (D’ignazio & Klein, 2020), in the short term our community has worked extensively to bring to light such issues. Concretely, much has been done to try and frame the problem, evaluate it and mitigate it.
% Having chiefly considered data as the main or even unique source of bias in NLP models, much work has a) analyzed which biases are exhibited in our corpora and to what extent. b) tried to mitigate bias by working on the data themselves (e.g. counterfactual data augmentation, fine-tuning on gender bias datasets). However, little attention has been given to other components of the models that exacerbate bias (Webster et al, 2020) 
% Another NLP line of research ( \〜interpretability) has tried to shed more light on our opaque models and other possible mechanisms that lead to bias outputs, for instance in pre-trained language models (Vig et al, 2020). In MT, bias-related work has focussed on NMT vs SMT algorithmic bias (Vanmassenhove, 2019), or on the inner linguistic representations of MT models (Bau et al, 2019), gender included.
% Closest to our intent are the works by (Costa Jussà et al, 2020) - which investigates the role different architectural designs play in gender bias in Multilingual MT - and (Roberts et al, 2020) proving that beam search is comparatively with sampling more biased toward the generation of more frequent (masculine) pronouns. In both works, it has been shown while “taken-for-granted” approaches, like -respectively - the use of Transformer architecture or beam search, improve overall translation quality in terms of BLUE scores, they are disadvantaged when it comes to gender bias. 
% Similarly, the BPE compression method is the MT state-of-the-art approach, and has been recently proved to be the highest-quality segmentation technique in ST as well (Di Gangi et al, 2020). But does it hold true for gender translation as well?

% gender agreement is a semantic and morphosyntactic phenomenon + several languages show complex feminine forms, typically derivative and created by adding a suffix to the masculine form, like Lehrer/Lehrerin(de), studente/studentessa(it). 
%  → statistical segmentation is limited with morphologically-rich  languages,  where  statistical  segmentation methods can break the morphological structure of words, losing relevant semantic and syntactic information.
% e.g. céléb r é vs celéb r é e
% Due to the under-representation of women in our datasets, and consequently of femininine forms ( 〜 data sparseness problem)--> statistical segmentation tends to leave unmerged less frequent words. 
% → maybe feminine words (being less frequent) receive different (unfavourable) segmentation
% e.g. H-9 des@@ crit@@ ta vs des@@ critto →  descritto and descritta are differently segmented

% Due to a) structural properties of feminine linguistic marking b) longer sequences of linguistically non-motivated tokens for feminine forms as a results of statistical segmentation: 
% models do not overgeneralize on certain forms?
% longer sequences are disadvantaged by beam search and not picked?

% We address these question by [SUMMARY OF EVAL SETTINGS]
% CONTRIBUTION: first analysis for both MT and ST in which 5 different segmentation techniques are compared in the light of gender bias + analysis 
% FINDINGS: [BLA]

